Mixed Reality UI Adaptations with Inaccurate and Incomplete Objectives

This position paper outlines a new approach to adapting 3D user interface (UI) layouts given the complex nature of end-user preferences. Current optimization techniques, which mainly rely on weighted sum methods, can be inflexible and result in unsatisfactory adaptations. We propose using multi-objective optimization and interactive preference elicitation to provide semi-automated, flexible, and effective adaptations of 3D UIs. Our approach is demonstrated using an example of single-element 3D layout adaptation with ergonomic objectives. Future work is needed to address questions around the presentation and selection of optimal solutions, the impact on cognitive load, and the integration of preference learning. We conclude that, to make adaptive 3D UIs truly effective, we must acknowledge the limitations of our optimization objectives and techniques and emphasize the importance of user control.

==> sections/notes.tex <==
\section{Notes}
\label{sec:notes}

\subsection{On Theory and Assumptions in Adaptive UI Research}

Our research --- and much of adaptive UI research for that matter --- tries to balance the same effectiveness-efficiency trade-off:
How can we best match end-user preferences (effectiveness) while requiring as little end-user effort as possible (efficiency)?
This formulation is underpinned by motivational, economic, and cognitive theory.
The end-user is assumed to be maximizing some kind of latent reward or utility (cf., for example, utility theory or computational rationality theory) which, somewhat imprecisely, may be thought of here as a form of satisfaction.\footnote{How this reward or utility may be operationalized or further understood is actually an active domain of research and is only simplified here for the sake of understandability.}
For illustration purposes, let us take here the perspective of computational rationality specifically --- a theory that has recently been proposed as a theory for interaction and computational interaction design.
Computational rationalit posits that end-users strive to maximize some kind of long-term reward $R$ (with future rewards discounted by some factor \gamma) by taking imperfect actions (i.e., approximately optimal actions corrupted by imperfect approximation and execution) based on imperfect information (i.e., based on optimality approximations corrupted by imperfect observation and inference).
Matching end-user preferences either in the short term (i.e., highly discounting future rewards) or long term (i.e., weakly discounting future rewards) is, then, assumed to contribute positively to these latent end-user rewards $R$ and, in turn, gives us such concrete adaptation formulations as moment-to-moment UI optimization based on approximate dynamic objectives (e.g., adapting a UI element's position in 3D during interactive usage based on pre-defined visibility objectives or timing notifications based on inference of current task or activity) or optimization at design time based on objectives related to long-term usage such as learnability and ergonomics (e.g., adapting a keyboard layout for improved ergonomics and learnability for a given language population).
Combinations of short and long-term optimization can equally be imagined where a UI is adapted online to maximize some long-term total utility with discounted future rewards (cf. MARLUI).
Interestingly, even such convincing long-term objectives as ergonomics may in fact only be assumed to contribute positively to end-user rewards, whereas users themselves may neither state their preferences for these long-term beneficial adaptations explicitly (e.g., prioritizing some short-term objective such as visibility over long-term health factors such as shoulder ergonomics) or implicitly (e.g., selecting a more convenient adaptation over a long-term benefical adapatation).
This phenomenon is widely known in such areas as workplace ergonomics (e.g., preferring to work in a comfortable arm chair over an ergonomic office chair) or addiction research (e.g., preferring to gamble despite its effects on long-term financial security or preferring to consume a toxic addictive substance despite its effects on long-term health).

End-user effort (as most often related to end-user input) is, conversely to matching end-user preferences, assumed to contribute negatively to the latent end-user rewards, either because of its implications on physical exertion (i.e., exerting energy to physically express opinions or preferences, for example, to select one potential adaptation over another) or mental demands (i.e., exerting energy to perceive, process and convey information, for example, to read a notification, to evaluate options, or to determine the best way to express one's opinions).
While these assumptions may be challenged in their own right --- end-user preferences may, for example, change in light of new information (e.g., based on an attempt to match some latent preference function) and may, as we have seen, poorly reflect actually beneficial outcomes for the user; end-user effort can be rewarding to the user in its own right (imagine, for example, the enjoyment derived from physical exhaustion in a fitness game or the (re-)evaluation of one's achievements based on the required "suffering" or challenge that is required reach these self-set goals (cf., for example, flow theory)) ---, the simplified framework laid out above holds for many current adaptive UI systems and techniques.
What is it then that differentiates adaptation approaches, besides the obvious application domain (e.g., text entry or 3D UI layout)?
It is how the specific adaptation technique tackles this effectiveness-efficiency trade-off.

Let us take an example.
The Adaptive User Interfaces Toolkit (AUIT) is a Unity-based UI adaptation framework that can be used to implement a variety of adaptation techniques for 3D UIs based on developer-defined objectives, adaptation triggers, and UI transitions.
It is remarkably flexible in its implementation.
As the authors note in AUIT's original publication, developers of adaptive mixed reality application can implement a variety of adaptation strategies and techniques and extend the existing components to create increasingly complex adaptive systems.
In its original implementation, AUIT utilizes a static weighted sum optimization based on developer-selected objectives to smoothly transition a 3D UI layout from one configuration to the next using animated spatial transformations.
The implicit assumption behind this setup is that the objectives chosen by the designer or developer are an appropriate approximation of the latent true preference criteria of the end-user and that their linear combination sufficiently matches the combination of these latent preference criteria in the end-user's latent true preference function.
It is further assumed that a single immediate adaptation is at least weakly preferred to (i.e., is as good as or better than) no adaptation (i.e., any adaptation computed by the system is at least as good as the current configuration given the new usage context).
It may even be argued that the system implicitly assumes that a single adaptation is weakly preferred to multiple adaptations (i.e., that translating and rotating the UI elements of the current configuration is at least as good as duplicating the UI elements at various points in the 3D space).
This may, however, only be a limitation of the system rather than an actual belief of its authors and AUIT can be extended to include adaptation to multiple configurations.
In light of the likely inaccuracy of the above approximations and assumptions, however, the system does not adapt fully automatically.
Instead, it queries the end-user (or the designer as a representative) in hope to increase its effectiveness at the cost of some efficiency.
In AUIT's original implementation, this query takes the form of the selection of objectives and the configuration of their weights.
End-users (or designers) are invited to customize the optimization's cost function to match their individual preferences given the specific application's usage context.
This introduces some friction to the otherwise fully automatic adaptation process.
In the framework established above, it aims to increase effectiveness at the cost of increased end-user (or designer) effort.
Similarly, allowing users to correct an adaptation (e.g., by dragging a UI element to reposition it), (re-)introduces some manual effort to the otherwise fully automatic adaptation procedure.
If the adaptations were truly optimal (i.e., the UI would adapt to at least one bundle of configurations that would be globally preferred), no reconfiguration would be required and, therefore, no affordances for manual repositioning.
It is thus that the system positions itself along the effectiveness-efficiency spectrum.
It sacrifices some efficiency, in terms of reintroducing end-user effort, to achieve higher levels of effectiveness with the overall goal to achieve maximum end-user satisfaction --- its substitute for that latent long-term end-user reward.
How do we then judge these adaptation techniques?
And how do we do so informed by theory and \textit{informing} theory along the way?
I propose that we take inspiration from closely related scientific communities such as in computational cognitive science and turn to an approach that has lead to tremendous advances in adaptive user interfaces and intelligent interfaces in general: explicit user modeling and simulation-based evaluation.

% Consequences for AUIT Pareto evaluation (if it is to be based in simulation): Define an interaction episode (POMDP) and implement a computational user model that has certain objectives (maybe a superset of the optimized objectives; e.g., also including some visual load metric) combined in some reward function, then let the user interact with the system and report the interaction episodes total reward
% Then, for an evaluation with real users, use one or a few highly rewarding adaptation system for the same interaction episode and ask them to rate their satisfaction (and maybe the criteria that the objectives were trying to model like visibility or reachability)
